Enhancing Data-Driven Reachability Analysis using Temporal Logic Side Information

This paper presents algorithms for performing data-driven reachability analysis under temporal logic side information. In certain scenarios, the data-driven reachable sets of a robot can be prohibitively conservative due to the inherent noise in the robot's historical measurement data. In the same scenarios, we often have side information about the robot's expected motion (e.g., limits on how much a robot can move in a one-time step) that could be useful for further specifying the reachability analysis. In this work, we show that if we can model this side information using a signal temporal logic (STL) fragment, we can constrain the data-driven reachability analysis and safely limit the conservatism of the computed reachable sets. Moreover, we provide formal guarantees that, even after incorporating side information, the computed reachable sets still properly over-approximate the robot's future states. Lastly, we empirically validate the practicality of the over-approximation by computing constrained, data-driven reachable sets for the Small-Vehicles-for-Autonomy (SVEA) hardware platform in two driving scenarios.

==> 6-reach_cont.tex <==

\subsection{Reachability Analysis for Continuous-Time Systems}

%To do, I think
%\begin{itemize}
%\item Introduce why this is a very interesting problem (discrete time measurements, but system continuous time)
%\item Introduce exact discretization (+ assumptions, if applicable)
%\item Explain the logm operator + its series calculation
%\item Motivate why this is a hard problem
%\item State assumption
%\item State Theorem + Proof
%\item Short remark that calculating the series with the zonotope is also possible with guaranteed approximation error, but numerics have shown that the results are overly conservative?
%\end{itemize}

We are interested in computing the reachable sets of continuous time systems that are consistent with the data sampled in discrete time. Consider the following state space
\begin{align}
    \dot{x}(t) = A_c x(t) + B_c u(t) + w(t). 
    \label{eq:syscont}
\end{align}

%Measuring the current is type of measuring the derivativeof the voltage of the capacitor. Also, measuring the voltage of the inductor is kind of measuring the derivative of the current. The accelerometer sensor is measuring the derivative of the velocity as well. This approach can be summarized in the following theorem and is useful in certain applications. 

We propose two approaches to compute these reachable sets. First approach requires collecting the derivative of the signal as done in \cite{conf:contin1,conf:contin2,conf:contin3} and one example for that is the accelerator sensor. If we consider sampled noisy state derivative $\tilde{\dot{x}}(k)$ and noisy state, i.e.,
\begin{align}
\tilde{\dot{x}}(k) = \dot{x}(k) + g(k),\\
\tilde{x}(k) = x(k) + v(k),
\end{align}

where $g(k) \in \mathcal{Z}_g=\zono{c_g,G_g}$ and $v(k) \in \mathcal{Z}_v$ are bounded measurement noise. We collect $T$ data points  
\begin{align*}
    \tilde{\dot{X}} &:= \begin{bmatrix} \tilde{\dot{x}}(0) & \tilde{\dot{x}}(1) & \dots & \tilde{\dot{x}}(T-1) \end{bmatrix},
\end{align*}
with noise
\begin{align*}
 \hat{G} &:= \begin{bmatrix} \hat{g}(0) & \hat{g}(1) & \dots &\hat{g}(T-1) \end{bmatrix}.
\end{align*}

Similar to before, we have the noise in the collected data within a matrix zonotope, i.e., $G \in \mathcal{M}_g =\zono{C_{\mathcal{M}_g},G_{\mathcal{M}_g}^{(1:T)}}$. The problem is close the noisy measurement for discrete system with additional noise $g(k) \in \mathcal{Z}_g$ that affects the derivative of the data. We have for specific data points with actual noise $\hat{g}(k)$, $\hat{v}(k)$ and $\hat{w}(k)$:

\begin{align}
    (\tilde{\dot{X}})_i - \hat{g}(k) = \begin{bmatrix} A_c & B_c \end{bmatrix} \begin{bmatrix} (\tilde{X}_-)_i \\ (U)_i \end{bmatrix} - A_c \hat{v}(k) + w(k).
\end{align}

Again we first fit a model $M_c$ while neglecting the term $A_c \hat{v}(k)$ using least square as follows:
\begin{align}
    M_c = (\tilde{X}_+ - C_{\mathcal{M}_g} - C_{\mathcal{M}_w}  ) D_c
    \label{eq:Mc}
\end{align}
where 
 \begin{align}
    \begin{bmatrix} 
    \tilde{X}_{-} \\ U_{-} 
    \end{bmatrix} D_c = I,
    \label{eq:cond2Mc}
\end{align}
Then we find a zonotope $\mathcal{Z}_d$ that bounds the term $AV_-$ and the model mismatch, with the assumption  that the data is informative enough, as follows

\begin{align}
    \mathcal{M}_d &=\dot{X} - \mathcal{M}_w - \mathcal{M}_g - M_c \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix}.\label{eq:zc}
    \end{align}
Then obtain the upper and lower bound in a zonotope $\mathcal{Z}_d$ from $\mathcal{M}_d$ as in \eqref{eq:argmaxMAV} and \eqref{eq:argminMAV}.  
    
%    \begin{align}
%[\underline{\mathcal{M}}_d , \overline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%(\overline{\mathcal{Z}_d})_i &= \argmaxB_j{(\overline{\mathcal{M}}_d)_{i,j}}, \\ (\underline{\mathcal{Z}_d})_i &= \argminB_j{(\underline{\mathcal{M}}_d)_{i,j}}, \\
%\mathcal{Z}_d &= \text{zonotope}(\underline{\mathcal{Z}}_d,\overline{\mathcal{Z}}_d). 
%\end{align}

Let $M_c =\begin{bmatrix} A_{M_c} & B_{M_c} \end{bmatrix}$. Then the next step is to use one of the readability analysis tool to find the reachable sets using the following parameters ($A_t$, $B_t$, $\mathcal{U}_t$, $\mathcal{X}_{t,0}$)
\begin{align}
 A_t &= A_{M_c}\\
 B_t & = 1 \\
 \mathcal{X}_{t,0} &= \mathcal{X}_{0} \\
 \mathcal{U}_t &= B_{M_c} \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
\end{align}

We consider the $\mathcal{Z}_w +\mathcal{Z}_d$ in $\mathcal{U}_t$ to be integrated along with the input. 

%\begin{theorem}
%Consider collected sampled data $\mathcal{D}$ from the system \eqref{eq:syscont}, the data-driven reachable set can be computed using traditional reachable techniques with the following parameters ($\mathcal{U}_c,\mathcal{A}_c,\mathcal{B}_c$)
%\begin{align}
% \mathcal{A}_c &= \mathcal{A}_{\Sigma,c}'\\
% \mathcal{B}_c & = 1 \\
% \mathcal{U}_c &= \mathcal{B}_{\Sigma,c}' \mathcal{U} + \mathcal{Z}_w +\mathcal{Z}_d
%\end{align}
%where
%\begin{align}
%\begin{bmatrix} 
%    X_- \\ U_- 
%\end{bmatrix} H &= I
%\end{align}
%\begin{align}
%\mathcal{M}_{\Sigma,c}' &= (\dot{X}_- - \mathcal{M}_w) H\\
%[ \mathcal{A}_{\Sigma,c}', \mathcal{B}_{\Sigma,c}'] &= \mathcal{M}_{\Sigma,c}'\\
%\mathcal{M}_d &=\dot{X}_- - \mathcal{M}_w - \mathcal{M}_{\Sigma,c} \begin{bmatrix}X_{-} \\ U_{-} \end{bmatrix},\label{eq:zc}\\
%[\overline{\mathcal{M}}_d , \underline{\mathcal{M}}_d ]&= \text{intervalMatrix}(\mathcal{M}_d),\\
%\overline{\mathcal{Z}_d}(i) &= \argmaxB_j{\overline{\mathcal{M}}_d(i,j)}, \\ \underline{\mathcal{Z}_d}(i) &= \argminB_j{\underline{\mathcal{M}}_d(i,j)}, \\
%\mathcal{Z}_d &= \text{zonotope}(\overline{\mathcal{Z}_d},\underline{\mathcal{Z}_d}), 
%\end{align}
%\end{theorem}



We propose another approach for data-driven reachability analysis for continuous time systems without requiring collecting the derivatives of the states. First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. Our approach is based on converting all the possible $\begin{bmatrix} A & B\end{bmatrix}$ in discrete time to continuous time. First we convert $\mathcal{M}_\Sigma$ to interval matrix which then bounds the all possible $\begin{bmatrix} A & B\end{bmatrix}$ as follows
\begin{align}
    [\underline{\mathcal{M}}_\Sigma,\overline{\mathcal{M}}_\Sigma ]&= intervalMatrix(\mathcal{M}_\Sigma) 
\end{align} 
 \begin{align}
   \underbrace{\begin{bmatrix}\underline{A} & \underline{B}\\ 0 & I\end{bmatrix}}_{\underline{D}} \leq \begin{bmatrix} A & B \\ 0 & I\end{bmatrix} \leq \underbrace{\begin{bmatrix} \overline{A} & \overline{B}   \\ 0 & I\end{bmatrix}}_{\overline{D}}
\end{align}  
where the operation $\leq$ is element wise. Let $\overline{D} = C_d + \Delta D_u$  and $\underline{D} = C_d - \Delta D_l$ where $C_d$ is any matrix between the bounds, i.e., $\underline{D} \leq C_d \leq \overline{D}$. The following theorem bounds all the possible $\begin{bmatrix} A_c & B_c\end{bmatrix}$ as follows: 

%Let $D_c :=  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}$, 

\begin{theorem}
Given the lower bounds $\begin{bmatrix}\underline{A} & \underline{B}\end{bmatrix}$ and upper bounds $\begin{bmatrix}\overline{A} & \overline{B}\end{bmatrix}$ on $\begin{bmatrix}A & B\end{bmatrix}$, we can bound $\begin{bmatrix}A_c & B_c\end{bmatrix}$ as follows
\begin{align}
   \begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix} \leq  \begin{bmatrix} A_c & B_c \\ 0 & I\end{bmatrix}  \leq \begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix}
\end{align}
\begin{align}
\begin{bmatrix} \overline{A}_c & \overline{B}_c \\ 0 & I\end{bmatrix} T_s&= \max(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix})\\
\begin{bmatrix} \underline{A}_c & \underline{B}_c \\ 0 & I\end{bmatrix}T_s &= \min(\log\begin{bmatrix} \overline{A} & \overline{B} \\ 0 & I\end{bmatrix},\log\begin{bmatrix} \underline{A} & \underline{B} \\ 0 & I\end{bmatrix}),
\end{align}
where $T_s$ is the sampling time, $0 \leq \Delta D_l \leq 1$, $0 \leq\Delta D_u \leq 1$, $\Delta D_l \leq (C_d-I)$, $\Delta D_u \leq (C_d-I)$, and $C_d - I \leq 1$. The log is the matrix logarithm. The max, min and less than are element wise. 
\end{theorem}




\begin{proof}
We aim to prove that we can still bound $\begin{bmatrix} A_c & B_c \end{bmatrix}$ given the bounds in discrete time. Taking the logarithm of a matrix of $C_d$ and represented by power series.
\begin{align}
     log(C_d) &= \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d - I)^k}{k}. \label{eq:cd}    %(C_d - I) - \frac{(C_d - I)(C_d - I)^T}{2}  +\dots
\end{align}
Considering $log(C_d +\Delta D)$ results in 
\begin{align}
log(C_d +\Delta D_u) =& \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(C_d  - I +\Delta D_u)^k}{k}\nonumber\\
=&  \sum_{k=1}^{\infty} \frac{(-1)^{k+1}}{k} \sum_{i=0}^{i}{k \choose i} (C_d  - I )^{k-i}\Delta D_u^i \label{eq:cddeltad}
%log(C_d +\Delta D) =& C_d +\Delta D - I - 0.5(C_d +\Delta D - I)^2 \nonumber\\
%&+ \frac{(C_d +\Delta D - I)^3}{3} - \frac{(C_d +\Delta D - I)^4}{4} + \dots \nonumber\\
%=&  C_d +\Delta D - I - 0.5 (C_d - I)^2 \nonumber\\
% - \Delta D (C_d  - I) - &0.5  \Delta D^2  + \frac{(C_d  - I)^3}{3} +  \Delta D(C_d  - I)^2 \nonumber\\ 
%+  \Delta D^2(C_d  - I) +& \frac{\Delta D^3}{3} - 0.25(C_d  - I)^4 - (C_d  - I)^3\Delta D \nonumber\\
%- 1.5(C_d  - I)^2&\Delta D^2 -  (C_d  - I)\Delta D^3 - 0.25 \Delta D^4 + \dots
\end{align}
Subtracting \eqref{eq:cd} from \eqref{eq:cddeltad} with denoting $h(\Delta D_u)= log(C_d +\Delta D_u) -  log(C_d)$ results in
\begin{align}
  h(\Delta D_u)\! =&\!\! \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} \bigg(\! \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\! \nonumber\\ 
  &+ (C_d  -\! I )^k\! \bigg) -  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k} (C_d  - I )^k \nonumber\\
   =& \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}\Delta D_u^i\!
\end{align}
Similarly, we can find $h(-\Delta D)$ as
\begin{align}
h(-\Delta D_l)\! =  \sum_{k=1}^{\infty}\frac{(-1)^{k+1}}{k}  \sum_{i=1}^{i}{k \choose i} (C_d  -\! I )^{k-i}(-\Delta D_l)^i
\end{align}
Bounding the system dynamics in continuous time can be done by making sure that both $h(\Delta D_u)$ and $h(-\Delta D_l)$ do not increase or decrease together but one increases and the other decreases. 
%\begin{align}
%log(C_d + \Delta D) - log(C_d)&= \Delta D - \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%+ \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 + \frac{\Delta D^3}{3} \nonumber\\
%- (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 - (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&\\
%log(C_d - \Delta D) - log(C_d)&= -\Delta D + \Delta D(C_d  - I) - 0.5\Delta D^2 \nonumber\\
%- \Delta D (C_d  - I)^2 +&  (C_d  - I)\Delta D^2 - \frac{\Delta D^3}{3} \nonumber\\
%+ (C_d  - I)^3\Delta D -& 1.5(C_d  - I)^2\Delta D^2 + (C_d  - I)\Delta D^3 \nonumber\\
%- \Delta D^4 + \dots&
%\end{align}
Given that $0 \leq \Delta D_u \leq 1$, $0 \leq \Delta D_l\leq 1$ and $(C_d-I) \leq 1$, then the dominant terms are $\Delta D_u$ and $\Delta D_u(C_d  - I)$ (similarly with $\Delta D_l$) and they are with different signs for $h(\Delta D_u)$ and $h(-\Delta D_l)$. At odd  value of index $i$, the $h(\Delta D_u)$ and $h(-\Delta D_l)$ have difference sign which support our claim. For index $i$ equals even values, both $h(\Delta D_u)$ and $h(-\Delta D_l)$ have the same sign. However given that $\Delta D_l \leq (C_d-I)$ and $\Delta D_u \leq (C_d-I)$, then there is always a term at the same index $i$ with greater value. %For instance, the terms $(C_d  - I)\Delta D^2$, $1.5(C_d  - I)^2\Delta D^2$, and $\Delta D^4$ are smaller than the comparable terms in the series.  
\end{proof}





%Assume that even though we have discrete-time trajectories, the underlying system is in fact continuous time. To retrieve a reachability analysis also in between data points, we are therefore interested in finding a set of continuous time systems that are consistent with the data.

%First of all, we assume that the discrete-time data points are obtained through zero-order hold inputs, which is the case in many application scenarios. % (note: realistic assumption on actuator). (Remark: This could also be refined to ramp-invariant transformation)





%Second assumption, we assume that the sampling rate is satisfactory and the spectral norm of $AT_s $ satisfies the following inequality:
%\begin{align*}
%   \| A T_s \| \leq 0.5
%\end{align*}

%Then we know 
%\begin{align*}
%    A_{\mathrm{disc}} &= e^{AT_s} = I + AT_s + \frac{1}{2!}(A T_s)^2 + \dots \\
%    B_{\mathrm{disc}} &= \int_0^{T_s} e^{At} B dt = \left( I T_s + A T_s^2 + \frac{1}{2!}A^2 T_s^3 + \dots \right) B
%\end{align*}

%\begin{theorem}
%The approximation error can be bounded by 
%\begin{align*}
%    \| E_m \| \leq \frac{\rho (L) ^{m+1}}{(m+1)(1+\rho(L))}
%\end{align*}
%where $\rho(L)$ denotes the spectral radius of $L$.
%\end{theorem}
%\begin{proof}
% (Lastman, Puthenpura and Sinha 1984)
%\end{proof}

%\subsubsection*{Algorithm \cite{conf:bookdisc2cont}}
%\begin{enumerate}
%    \item Determine $L = A_{\mathrm{disc}} - I$.
%    \item Set $D^{(1)} = I$, $M^{(1)} = I$ and $i=1$.
%    \item Perform the following computations recursively
%    \begin{align*}
%        M^{(i+1)} &= \frac{-i L M^{(i)}}{i+1} \\
%        D^{(i+1)} &= D^{(i)} + M^{(i+1)} \\
%        i &= i+1
%    \end{align*}
%    until $i=m$.
%    \item Finally, $AT = DL$, $BT = D B_{\mathrm{disc}}$
%\end{enumerate}



% This is what we need!
% https://link.springer.com/content/pdf/10.1007%2F978-94-011-3558-0.pdf p.131

%A method to calculate \cite{conf:disc2cont}, but calculations are involved and not tractable for matrix zonotopes. However, we can calculate the Euler approximation and then bound the local truncation error?

% Can we use this? "TRANSFORMATION OF CONTINUOUS-TIME MODEL OF A LINEAR MULTIVARIABLE SYSTEM FROM ITS DISCRETE-TIME MODEL"

%\tb{no results here - just thoughts we can discuss}
%$\rightarrow$ How can we find the continuous time state space description?
%Assuming zero-order hold for the input (I think a good choice), we retrieve
%\begin{align*}
%    A_{\text{disc}} = e^{AT_s}
%\end{align*}
%with $T_s$ being the sampling time. However, calculating the logarithm of a matrix is usually done via diagonalization. If $\|A_{\text{disc}} - I \| < 1$ (what does that mean for us?), then it can be calculated the following series converges:
%\begin{align*}
%    A T_s = \log (A_{\mathrm{disc}}) = \sum_{k=1}^{\infty} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}
%\end{align*}
%..can we calculate this sum via Zonotopes? We can only be approximating the true matrix.

%..which is actually the Euler integration. For small timesteps $T_s$, $e^{A T_s} \approx I + A T_s $, i.e. $A T_s \approx A_{\mathrm{disc}} - I  \left( = \sum_{k=1}^{1} (-1)^{k+1} \frac{(A_{\mathrm{disc}} - I)^k}{k}\right)$, $B T_s \approx B_{\mathrm{disc}}$. % $D_{\mathrm{disc}} = D$, $C_{\mathrm{disc}} = C$
% http://eceweb1.rutgers.edu/~gajic/solmanual/slides/chapter8_DIS.pdf
% https://homes.esat.kuleuven.be/~maapc/static/files/CACSD/Slides/chapter2.pdf

%I guess we can use Euler discretization for small timesteps - but we introduce an error. Can we bound the error? Then we could add this error in the reachability analysis. 

%The local error (error per step) is proportional to the square of the step size.
%Assume $x$ has a continuous second derivative. Local truncation error LTE:
%\begin{align*}
%    \mathrm{LTE} = \frac{1}{2} T_s^2 M 
%\end{align*}
%where $M$ is the an upper bound on the second derivative of $x$ on the given interval $[t_0, t_0 + h]$.

%\begin{align*}
%    \dot{x} &= Ax + Bu \\
%    \ddot{x} &= A \dot{x} = A^2 x + ABu
%\end{align*}
%While we cannot calculate the exact discretization error, we can approximate it by $A_{\mathrm{disc}}^2 x(t_0) + A_{\mathrm{disc}} B_{\mathrm{disc}} u(t_0)$? \tb{tbd}.





%Let $\mathcal{M}_{\Sigma} = \begin{bmatrix}\mathcal{M}_{\Sigma A} & \mathcal{M}_{\Sigma B} \end{bmatrix}$. The reachable region can be over approximated by 
%\begin{align}
%\mathcal{R}_{k+1} = \mathcal{M}_{\Sigma A} \mathcal{R}_{k} + \mathcal{M}_{\Sigma B} \mathcal{U} +  \mathcal{M}_w
%\end{align}
%
